All centralising monoids with majority witnesses on a four-element set

We study unary parts of centraliser clones on the set $\{0,1,2,3\}$, so-called centralising monoids. We describe and count all centralising monoids on the set $\{0,1,2,3\}$ having majority operations as witnesses, and we list the inclusion maximal proper submonoids of the full transformation monoid among them. This extends previous work by Goldstern, Machida and Rosenberg.

==> hyphexcept.tex <==
%1 vim: set ft=tex:
%2 Use ./sorthyph.sh to bring this file in alphabetical order.
%3 This is essentially the command `sort -d -f'.
\hyphenation{an-aly-ses}
\hyphenation{an-aly-sis}
\hyphenation{as-so-cia-tive}
\hyphenation{as-so-cia-tiv-ity}
\hyphenation{auto-morph-ic}% (2!)
%\hyphenation{auto-morph-ism}% okay
%\hyphenation{auto-morph-isms}% okay
\hyphenation{au-tono-mous}
\hyphenation{au-tono-mous-ly}% (2!)
\hyphenation{be-tween}
\hyphenation{Bool-ean}
\hyphenation{bound-ed}% (2!)
\hyphenation{Car-te-sian}
%\hyphenation{cat-e-go-ries} %AE??
%\hyphenation{cat-egor-ies}% okay
\hyphenation{com-mu-ta-tive}
\hyphenation{com-mu-ta-tiv-ity}
\hyphenation{con-se-quence}
\hyphenation{con-se-quences}
\hyphenation{con-se-quent-ly}% (2!)
\hyphenation{Con-se-quent-ly}% (2!)
\hyphenation{co-ord-in-ate}
\hyphenation{def-in-ition}
\hyphenation{Def-in-ition}
\hyphenation{def-in-itions}
\hyphenation{Def-in-itions}
\hyphenation{de-ter-mine}
\hyphenation{de-ter-mined}
\hyphenation{de-ter-mined-ly}% (2!)
\hyphenation{de-ter-min-ing}
\hyphenation{endo-morph-ic}% (2!)
\hyphenation{endo-morph-ism}
\hyphenation{endo-morph-isms}
\hyphenation{equiva-lence}
\hyphenation{equiva-lences}
\hyphenation{equiva-lent}
\hyphenation{equiva-lent-ly}% (2!)
\hyphenation{homeo-morph-ic-al-ly}% (!2)
\hyphenation{Homeo-morph-ic-al-ly}% (!2)
\hyphenation{homeo-morph-ic-ity}%
\hyphenation{Homeo-morph-ic-ity}%
%\hyphenation{homeo-morph-ism}% okay
%\hyphenation{homeo-morph-isms}% okay
\hyphenation{idem-po-tents}
\hyphenation{idem-po-tent}% see po-tent
\hyphenation{iden-ti-cal}
\hyphenation{im-pli-ca-tion}
\hyphenation{Im-pli-ca-tion}
\hyphenation{im-pli-ca-tions}
\hyphenation{Im-pli-ca-tions}
\hyphenation{ir-re-du-ci-bil-ity}
%%\hyphenation{ir-re-duc-ibil-i-ty}% AE?
%%\hyphenation{ir-re-duc-ible}% AE?
%\hyphenation{ir-re-du-cible}% okay
%\hyphenation{ir-re-du-cibly}% okay
\hyphenation{iso-morph-ic} % last hyphen probably not recognised due to
%\hyphenation{iso-morph-ism}% okay
%\hyphenation{iso-morph-isms}% okay
\hyphenation{lem-ma}% (2!) % BE: not at all
\hyphenation{Lem-ma}% (2!) BE: not at all
\hyphenation{more-over}
\hyphenation{More-over}
\hyphenation{neigh-bour-hood}
\hyphenation{neigh-bour-hoods}
\hyphenation{non-au-tono-mous}
\hyphenation{poly-morph-ic}% (!2)
%\hyphenation{poly-morph-ism}% okay
%\hyphenation{poly-morph-isms}% okay
\hyphenation{posi-tive-ly}% (!2)
\hyphenation{prod-uct}
\hyphenation{prod-ucts}
\hyphenation{re-la-tion-al}% (2!)
\hyphenation{re-la-tion-al-ly}% (2!)
\hyphenation{semi-group}
\hyphenation{semi-groups}
\hyphenation{semi-lat-tice}
\hyphenation{semi-lat-tices}
\hyphenation{strength-en}% (2!)
\hyphenation{strength-ened}
\hyphenation{tauto-logic-al}% (2!)
\hyphenation{tauto-logic-al-ly}% (2!)
\hyphenation{tau-tolo-gies}
\hyphenation{tau-tolo-gous}
\hyphenation{tau-tol-ogy}
\hyphenation{topo-logic-al}% (2!)
\hyphenation{topo-logic-al-ly}% (2!)
\hyphenation{top-olo-gies}
\hyphenation{Top-olo-gies}
\hyphenation{top-ology}
\hyphenation{Top-ology}
\hyphenation{when-ever}

